Tracking Network Events with Write Optimized Data Structures: The Design and Implementation of TWIAD: The Write-Optimized IP Address Database

Access to network traffic records is an integral part of recognizing and addressing network security breaches. Even with the increasing sophistication of network attacks, basic network events such as connections between two IP addresses play an important role in any network defense. Given the duration of current attacks, long-term data archival is critical but typically very little of the data is ever accessed. Previous work has provided tools and identified the need to trace connections. However, traditional databases raise performance concerns as they are optimized for querying rather than ingestion. The study of write-optimized data structures (WODS) is a new and growing field that provides a novel approach to traditional storage structures (e.g., B-trees). WODS trade minor degradations in query performance for significant gains in the ability to quickly insert more data elements, typically on the order of 10 to 100 times more inserts per second. These efficient, out-of-memory data structures can play a critical role in enabling robust, long-term tracking of network events. In this paper, we present TWIAD, the Write-optimized IP Address Database. TWIAD uses a write-optimized B-tree known as a B {\epsilon} tree to track all IP address connections in a network traffic stream. Our initial implementation focuses on utilizing lower cost hardware, demonstrating that basic long-term tracking can be done without advanced equipment. We tested TWIAD on a modest desktop system and showed a sustained ingestion rate of about 20,000 inserts per second.

==> dataset.tex <==
We used the publicly available backscatter dataset from the Center for Applied Internet Data
Analysis (CAIDA)~\cite{backscatter}. This dataset is essentially random so this is the worst case 
we will see in the real world. 

The dataset consists of collections of responses to spoofed traffic sent by denial-of-service attack victims and 
received by the UC San Diego (UCSD) Network Telescope. Data was collected between 2001 and 2008.

\iffalse

In these traffic traces destinations on the UCSD Network Telescope are anonymized 
by zeroing the first octet of the IP address. The source addresses (representing 
denial-of-service attack victims) were not modified.

When a denial-of-service-attack victim receives attack traffic with spoofed source IP addresses, 
the attack victim cannot differentiate between this spoofed traffic and legitimate requests, 
so the victim replies to the spoofed source IP addresses. These spoofed IP addresses were not the 
actual sources of the attack traffic, so they receive responses to traffic they never sent. 
By measuring this response traffic to a large portion of IP addresses (roughly a /8 network), 
it is possible to estimate a lower bound for the overall volume of spoofed source denial-of-service attacks occurring on the Internet.

The collections were made on:
\begin{itemize}
 \item 2001: February 2 to August 15
 \item 2002: May 9 to June 15, December 11 to 19
 \item 2003: November 6 to November 11
 \item 2004: February 25 to March 6, May 26 to June 3, August 26 to September 3, November 24 to December 2
 \item 2005: February 23 to March 3, May 25 to June 2, August 24 to September 1, November 23 to December 1
 \item 2006: February 22 to March 2, May 24 to June 1, August 23 to 31, November 22 to 30
 \item 2007: January 8 to 11, February 21 to March 1, May 23 to 31, August 23 to 30, November 20 to 29
 \item 2008: February 20 to 28, March 18 to 19, May 21 to 29, August 20 to 28, November 12 to 19
\end{itemize}

We used the data for \hxnt{TODO: Fill in what dates we used (large/small).}

The data from CAIDA is in the form of packet captures (PCAPs) --- we processed these PCAPs through Bro,
a network traffic analysis system~\cite{bro, paxson1999bro}. The PCAPs were converted into Bro connection logs which sessionize
the data and generates one row per network connection.

\hxnt{TODO: stats script for the following info on large/small}
Number of files,
number of entries (events). General understanding statistics of the data.
Use some diagrams 
\begin{enumerate}
  \item timestamp range
 \item burst data
 \item IP frequency histograms
 \item Port frequency histograms / lists
 \item Duration statistics - hist, mean, max, etc.
 
\end{enumerate}
\fi
